Dialog Structure Through the Lens of Gender, Gender Environment, and Power

Understanding how the social context of an interaction affects our dialog behavior is of great interest to social scientists who study human behavior, as well as to computer scientists who build automatic methods to infer those social contexts. In this paper, we study the interaction of power, gender, and dialog behavior in organizational interactions. In order to perform this study, we first construct the Gender Identified Enron Corpus of emails, in which we semi-automatically assign the gender of around 23,000 individuals who authored around 97,000 email messages in the Enron corpus. This corpus, which is made freely available, is orders of magnitude larger than previously existing gender identified corpora in the email domain. Next, we use this corpus to perform a large-scale data-oriented study of the interplay of gender and manifestations of power. We argue that, in addition to one's own gender, the "gender environment" of an interaction, i.e., the gender makeup of one's interlocutors, also affects the way power is manifested in dialog. We focus especially on manifestations of power in the dialog structure --- both, in a shallow sense that disregards the textual content of messages (e.g., how often do the participants contribute, how often do they get replies etc.), as well as the structure that is expressed within the textual content (e.g., who issues requests and how are they made, whose requests get responses etc.). We find that both gender and gender environment affect the ways power is manifested in dialog, resulting in patterns that reveal the underlying factors. Finally, we show the utility of gender information in the problem of automatically predicting the direction of power between pairs of participants in email interactions.

==> header.tex <==
\newcommand{\thesistitle}{Social Power in Interactions:\\ Computational Analysis and Detection of Power Relations}


\newcommand{\thesisauthor}{Vinodkumar Prabhakaran}
\newcommand{\thesisyear}{2015}



\usepackage[dvips]{epsfig}
\usepackage{amsmath}
\usepackage{fancyhdr}
\usepackage{afterpage}


\paperwidth=8.5in
\paperheight=11in

\setlength{\hoffset}{0.0in}
\setlength{\oddsidemargin}{0.25in}
\setlength{\textwidth}{6in}
\setlength{\evensidemargin}{0mm}

\setlength{\voffset}{0.0in}
\setlength{\topmargin}{.0in}
\setlength{\headheight}{14pt}
\setlength{\headsep}{22pt}
\setlength{\textheight}{8.5in}
\setlength{\footskip}{0pt}




\newcommand{\singlespace}{\renewcommand{\baselinestretch}{1.15} \small \normalsize}
\newcommand{\oneandhalfspace}{\renewcommand{\baselinestretch}{1.3} \small \normalsize}
\newcommand{\doublespace}{\renewcommand{\baselinestretch}{1.5} \small \normalsize}
\newcommand{\normalspace}{\doublespace}
\footnotesep=1\baselineskip

\setcounter{secnumdepth}{3}
\setcounter{tocdepth}{3}

\newcommand{\thesistitlepage}{
    \normalspace
    \thispagestyle{empty}
    \begin{center}
        \textbf{\LARGE \thesistitle} \\[1cm]
        \textbf{\LARGE \thesisauthor} \\[8cm]
        Submitted in partial fulfillment of the \\
        requirements for the degree \\
        of Doctor of Philosophy \\
        in the Graduate School of Arts and Sciences \\[4cm]
        \textbf{\Large COLUMBIA UNIVERSITY} \\[5mm]
        \thesisyear
    \end{center}
    \clearpage
}

\newcommand{\thesiscopyrightpage}{
    \thispagestyle{empty}
    \strut \vfill
    \begin{center}
      \copyright \thesisyear \\
      \thesisauthor \\
      All Rights Reserved
    \end{center}
    \cleardoublepage
}

\newcommand{\thesisabstract}{
    \thispagestyle{empty}
    \begin{center}
    \textbf{\LARGE ABSTRACT} \\[1cm]
     \textbf{\LARGE \thesistitle} \\[1cm]
     \textbf{\LARGE \thesisauthor} \\[1cm]
    \end{center}
    \input{inputs/abstract}
    \cleardoublepage
}

\newcommand{\draft}{
    \renewcommand{\normalspace}{\singlespace}
    \normalspace
    \chapter*{Draft. Version \today}
\clearpage }


==> todo.tex <==
\section*{To Do List}


\begin{itemize}
	\item Rewrite the abstract more generally. Pitch it in the beginning more in terms of why is this important, than starting with what we did. 
	\item Fix all chapter, section references (DONE)
	\item Add more references to computational work on gender in the last year in section 2.3
	\item Add the info about Data in section 3. Currently it refers back to the Data chapter in the thesis. 
\end{itemize}

\newpage


